Precise one-dimensional nanochannels in transition metal dichalcogenides as building blocks for advanced nanophotonics

Atomically sharp edges are essential for future high-index nanophotonic structures, yet conventional lithography and dry etching methods inevitably introduce edge roughness that limits optical confinement and reproducibility. Recently, anisotropic wet etching of multilayer van der Waals crystals, such as transition metal dichalcogenides (TMDs), has enabled crystallographically defined, atomically sharp zigzag edges, eliminating the edge-roughness problem. However, the process is intrinsically limited to confined geometries such as isolated triangular or hexagonal features dictated by crystal stacking symmetry. Here, we demonstrate a lithography-guided anisotropic etching framework that drives TMDs etching beyond isolated confined geometries by enforcing controlled interaction of neighboring etched nanoholes regions. In multilayer 2H-WS2, merging of anisotropic etch fronts enables sustained long-range propagation of zigzag facets, introducing a previously inaccessible 180-degree edge alignment and a crystallographically defined design space combining 120-degree and 180-degree junctions. Using this approach, we fabricate extended nanophotonic structures with ultrasharp sidewalls, including sub-100-nm-gap one-dimensional gratings, waveguides, defect-engineered photonic cavities, angle programmed photonic lattices, and diffractive zone plates. Back-focal-plane reflection spectroscopy of atomically sharp 1D periodic 2H-WS2 gratings demonstrates their photonic functionality, revealing symmetry-protected bound states in the continuum (SP-BICs) and strong exciton-photon coupling in multilayer WS2. Finally, we fabricate ultrathin, ultranarrow, and ultralong nanoribbons with record-high aspect ratios. Together, these results demonstrate edge merging as a generic route to fabricate edge-defined, atomically sharp nanophotonic and nanoelectronic architectures in layered van der Waals platforms.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
